VideoScore2: Think before You Score in Generative Video Evaluation

Recent advances in text-to-video generation have produced increasingly realistic and diverse content, yet evaluating such videos remains a fundamental challenge due to their multi-faceted nature encompassing visual quality, semantic alignment, and physical consistency. Existing evaluators and reward models are limited to single opaque scores, lack interpretability, or provide only coarse analysis, making them insufficient for capturing the comprehensive nature of video quality assessment. We present VideoScore2, a multi-dimensional, interpretable, and human-aligned framework that explicitly evaluates visual quality, text-to-video alignment, and physical/common-sense consistency while producing detailed chain-of-thought rationales. Our model is trained on a large-scale dataset VideoFeedback2 containing 27,168 human-annotated videos with both scores and reasoning traces across three dimensions, using a two-stage pipeline of supervised fine-tuning followed by reinforcement learning with Group Relative Policy Optimization (GRPO) to enhance analytical robustness. Extensive experiments demonstrate that VideoScore2 achieves superior performance with 44.35 (+5.94) accuracy on our in-domain benchmark VideoScore-Bench-v2 and 50.37 (+4.32) average performance across four out-of-domain benchmarks (VideoGenReward-Bench, VideoPhy2, etc), while providing interpretable assessments that bridge the gap between evaluation and controllable generation through effective reward modeling for Best-of-N sampling. Project Page: https://tiger-ai-lab.github.io/VideoScore2/

==> tables/3_IAA.tex <==
\begin{wraptable}{r}{0.43\textwidth}
    \small
    \centering
    % \renewcommand{\arraystretch}{1.2}
    \caption{Inter-Annotator Agreement (IAA) analysis results.}
    \scalebox{0.9}{
    \setlength{\tabcolsep}{6pt}
    \begin{tabularx}{0.9\linewidth}{l|ccc}
    \toprule
    IAA metric  & VQ    & TA    & PC     \\
    \midrule
    \multicolumn{4}{c}{Trial 1 (\#=30)}                  \\
    \midrule
    Relaxed Match  &  &  &  \\
    SPCC       &  &  &  \\
    Alpha       &  &  &  \\
    \midrule
    \multicolumn{4}{c}{Trial 2 (\#=50)}   \\
    \midrule
    Relaxed Match &  &  &  \\
    SPCC       &  &  &  \\
    Alpha       &  &  &  \\
    \bottomrule
    \end{tabularx}
    }
    
    \label{tab:3_IAA}
    \vspace{-4pt}
\end{wraptable}

==> tables/3_score_difference.tex <==
% \begin{wraptable}{r}{0.53\textwidth}
%     \small
%     \centering
%     % \renewcommand{\arraystretch}{0.6}
%     
%     \caption{Human inspection on the difference between model score and human score in augmented-scoring.}
%     \label{tab:3_score_diff_dist}
% \end{wraptable}



\begin{wraptable}{r}{0.43\textwidth}
    \small
    \centering
    \renewcommand{\arraystretch}{1.3}
    \caption{Human inspection on the difference between model score and human score in augmented-scoring.}
    \scalebox{0.87}{
    \begin{tabularx}{0.98\linewidth}{l|cccc}
    \toprule
    \multicolumn{5}{c}{\textbf{4951} videos, \textbf{14853} scores in total} \\
    \midrule
    Difference  & 0 & 1 & 2 & $\geq$3 \\
    \midrule 
    Counts & 4710 & 7698 & 2062 & 383 \\
    \midrule
    \multicolumn{5}{c}{Bad videos (diff. $\geq$3 in any dim.) : \textbf{337 / 4951}}   \\
    \bottomrule
    \end{tabularx}
    }
    
    \label{tab:3_score_difference}
\end{wraptable}

==> tables/_discard__4_ablation.tex <==
\begin{table}[h]

\small
\centering
\setlength{\tabcolsep}{5pt}
\caption{Ablations on rationale in SFT, w/o SFT removes evaluation thinking process in training data and instructs the video to give score only.}
\scalebox{0.83}{
\renewcommand{\arraystretch}{1.25}

\begin{tabular}{l|ccc|c|ccc|c|ccc|c}
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{Relaxed Accuracy} & \multicolumn{4}{c}{PLCC}  \\  \cmidrule{2-13}
 & Visual  & Align  & Phy  & Avg  
 & Visual  & Align  & Phy  & Avg    
 & Visual  & Align  & Phy  & Avg  \\ 
\midrule
w/ rationale & 47.00 & 42.60 & 38.40 & 42.67 & 93.60 & 87.20 & 86.00 & 88.93 & 56.74 & 58.24 & 44.72 & 53.23 \\

w/o rationale & 34.20 & 36.40 & 25.90 & 32.17 & 79.20 & 78.20 & 70.60 & 76.00 & 64.25 & 63.12 & 56.26 & 61.21 \\

\bottomrule
\end{tabular}
}


\label{tab:4_ablation}
\end{table}

==> tables/_discard__4_ood_bench_all.tex <==
\renewcommand{\arraystretch}{1.25}
\begin{table}[ht]
\small
\centering


\caption{Performance comparison on out-of-domain benchmarks, with 3 pairwise preference benchmarks and 3 point-score benchmarks. \textbf{Bold} denotes the best model and the \underline{underlined} denotes the second best.}
\scalebox{0.70}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cc|cc|cc|ccc|ccc}
\toprule
 & \multicolumn{6}{c|}{\textbf{OOD Preference Benchmark}}  & \multicolumn{3}{c|}{\textbf{OOD Point Score Benchmark}} & \multicolumn{3}{c}{\textbf{Average}}  
 \\ \cmidrule(lr){2-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
\multirow{2}{*}{} & \multicolumn{2}{c}{\textbf{VideoGen-}}    & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{GenAI-Bench}}} & \multicolumn{2}{c|}{\textbf{T2VQA-DB}}     & \textbf{MJ-Bench}    & \textbf{VideoPhy2}     & \textbf{AIGVE}      & \multirow{3}{*}{\textbf{w/ ties}} & \multirow{3}{*}{\textbf{w/o ties}} & \multirow{3}{*}{\textbf{both}} \\
 & \multicolumn{2}{c}{\textbf{Reward Bench}} & \multicolumn{2}{c}{}   & \multicolumn{2}{c|}{\textbf{(Preference)}} & \textbf{-Video}    & \textbf{-test}      & \textbf{-Bench}     &                            &                           &                       \\ 
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}
   & w/ ties  & w/o ties & w/ ties  & w/o ties  & w/ ties  & w/o ties & Overall & Averaged & Averaged & & &    \\ 
\midrule
\multicolumn{13}{c}{\textbf{Reward/Scoring Models for Image} (averaged on sampled frames)} \\ 
\midrule
ImageReward & 47.14 & 58.61 & 47.42 & 70.57 & 43.46 & 52.93 & 37.51 & 21.48 & 28.16 & 37.53 & 44.88 & 45.25 \\
DeQA-Score  & 53.88 & 67.91 & 44.95 & 66.96 & 35.22 & 55.47 & 44.19 & 28.85 & 22.60 & 38.28 & 47.66 & 46.67 \\
Q-Insight  & 54.05 & 66.34 & 46.08 & 68.73 & 46.65 & 51.84 & 52.58 & 30.90 & 23.91 & 42.36 & 49.05 & 49.01 \\
\midrule
\multicolumn{13}{c}{\textbf{Reward/Scoring Models for Video}} \\ 
\midrule
VideoScore-v1.1 & 16.79 & 40.19 & 32.96 & 49.88 &  39.18 & 39.24 & 71.57 & 27.95 & 21.51 & 34.99 & 41.72 & 33.84 \\
VideoReward     & 59.69 & 73.66 & 46.77 & 70.34 & 36.15 & 61.85 & 51.75 & 31.33 & 21.82 & 41.25 & 51.79 & 50.37 \\
UnifiedReward   & 53.31 & 58.83 & 49.29 & 63.70 & 50.39 & 51.96 & 23.18 & 22.02 & 47.88 & 41.01 & 44.59 & 46.73 \\
VisionReward    & 54.31 & 67.58 & 50.16 & 72.41 & 37.64 & 56.90 & 56.91 & 22.58 & 25.99 & 41.26 & 50.39 & 49.39 \\
Q-Align         & 42.05 & 52.52 & 45.16 & 67.20 & 43.24 & 51.84 & 21.97 & 23.22 & 32.10 & 34.62 & 41.47 & 42.14 \\
LiFT            & 32.80 & 29.93 & 33.48 &  9.48 & 13.74 & 10.76 & 15.47 &   --  & 41.08 & 27.31 & 21.34 & 23.34 \\
AIGVE-MACS      & 37.09 & 37.08 & 37.69 & 35.38 & 36.91 & 36.52 & 31.00 & 16.93 & 53.44 & 35.51 & 35.06 & 35.78 \\
VideoPhy2       & 30.75 & 26.41 & 35.65 & 27.19 & 24.12 & 21.86 & 24.00 & 37.64 & 49.59 & 33.62 & 31.11 & 30.80 \\
Dover           & 54.27 & 68.58 & 44.79 & 67.76 & 44.62 & 53.11 & 43.69 & 28.21 & 27.43 & 40.50 & 48.13 & 48.05 \\

\midrule
\multicolumn{13}{c}{\textbf{Ours}} \\ 
\midrule
\score (SFT only) &  &  & 41.56 & 63.59 & 52.36 & 59.32 & 66.88 & 30.31 & 34.83 &  &  &  \\
\score (RL w/o SFT) & & & & & & & & & & & & \\
\score (SFT\ +\ RL) & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
}

\vspace{-8pt}
\label{tab:4_ood_bench_all}
\end{table}

==> tables/_discard__4_vs2_bench_all_metrics.tex <==
\begin{table}[h]

\small
\centering
\caption{Accuracy and correlation between model answer and human score on \bench. \textbf{Bold} denotes the best model and the \underline{underlined} denotes the second best.}
\scalebox{0.67}{
\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|c|ccc|c|ccc|c|ccc|c}
\toprule

\multirow{2}{*}{} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{Relaxed Accuracy} & \multicolumn{4}{c|}{SPCC} & \multicolumn{4}{c}{PLCC} \\  \cmidrule{2-17}
    & Visual & Align & Phy & Avg  
    & Visual & Align & Phy & Avg    
    & Visual & Align & Phy & Avg 
    & Visual & Align & Phy & Avg \\ \midrule
Random & 19.57 & 19.57 & 18.44  & 19.19 & 56.51 & 56.65 & 57.65 & 56.94 & -0.04 & 0.11 & -1.28 &  -0.41 & -0.07 & 0.46 & -0.51 & -0.31 \\ 
\midrule
\multicolumn{17}{c}{\textbf{Prompting MLLM} (with same template)} \\ 
\midrule
Claude-Sonnet-4 & 33.07 & 29.86 & 23.85 & 28.93 & 76.35 & 76.95 & 61.92 & 71.74 & 17.15 & 30.29 & 16.31 & 21.25 & 20.17 & 30.64 & 18.01 & 22.94 \\
Gemini-2.5-Pro & 29.92 & 29.72 & 24.07 & 27.90 & 71.49 & 70.88 & 61.45 & 67.94 & 26.92 & 33.33 & 22.38 & 27.54 & 26.71 & 32.96 & 19.75 & 26.47 \\
GPT-5 & 30.72 & 27.91 & 20.08 & 26.24 & 73.90 & 72.29 & 60.84 & 69.01 & 11.85 & 23.09 & 16.42 & 17.12 & 13.38 & 23.34 & 17.24 & 17.99 \\
Gemini-2.5-Flash & 28.17 & 22.33 & 23.14 & 24.55 & 69.62 & 60.56 & 58.95 & 63.04 & 22.63 & 25.70 & 27.61 & 25.31 & 23.82 & 26.29 & 26.97 & 25.69 \\
o4-mini & 29.66 & 26.45 & 13.82 & 23.31 & 75.15 & 70.14 & 46.09 & 63.79 & 23.43 & 28.00 & 14.09 & 21.84 & 24.59 & 28.16 & 11.46 & 21.40 \\
Grok-4 & 21.01 & 23.53 & 18.07 & 20.87 & 64.29 & 62.82 & 55.25 & 60.79 & 6.90 & 13.10 & 6.28 & 8.76 & 8.11 & 12.66 & 6.51 & 9.09 \\
GLM-4.1v-9B-Thinking & 33.27 & 31.46 & 21.42 & 28.72 & 80.76 & 77.15 & 61.22 & 73.04 & 26.85 & 13.03 & 10.00 & 16.63 & 28.03 & 16.80 & 10.18 & 18.34 \\
GLM-4.5v & 29.72 & 28.51 & 20.08 & 26.10 & 73.49 & 70.68 & 55.22 & 66.46 & 12.87 & 15.04 & 9.45 & 12.45 & 14.39 & 15.37 & 10.73 & 13.50 \\
Qwen2.5-VL-72B-Instruct & 28.84 & 27.91 & 19.07 & 25.27 & 72.33 & 77.21 & 55.58 & 68.37 & 9.26 & 6.65 & 0.05 & 5.32 & 14.51 & 6.63 & 0.85 & 7.33 \\
Llama-4-Scout & 21.84 & 26.45 & 16.63 & 21.64 & 57.11 & 68.34 & 48.10 & 57.85 & -0.55 & 11.05 & 5.08 & 5.19 & 2.11 & 10.88 & 6.31 & 6.43 \\
Llama-4-Maverick & 26.25 & 24.25 & 18.04 & 22.85 & 62.73 & 68.54 & 48.50 & 59.92 & 3.53 & 9.60 & 9.19 & 7.44 & 4.97 & 10.55 & 6.74 & 7.42 \\


\midrule
\multicolumn{17}{c}{\textbf{Reward/Scoring Models for Image} (averaged on sampled frames)} \\ \midrule
ImageReward        & 29.06 & 28.06 & 27.26 & 28.13 & 65.13 & 68.94 & 61.72 & 65.26 & 24.46 & 35.89 & 21.31 & 27.22 & 28.23 & 40.76 & 23.26 & 30.75 \\
DeQA               & 36.87 & 28.66 & 32.06 & 32.53 & 85.37 & 77.15 & 80.96 & 81.16 & 37.51 & 15.88 & 26.21 & 26.53 & 44.87 & 23.96 & 29.73 & 32.85 \\
Q-Insight          & 33.60 & 30.60 & 31.00 & 31.73 & 81.40 & 77.40 & 75.60 & 78.13 & 33.32 & 18.28 & 22.96 & 24.85 & 41.05 & 25.44 & 27.54 & 31.34 \\
\midrule
\multicolumn{17}{c}{\textbf{Reward/Scoring Models for Video}} \\ 
\midrule
VideoScore-v1.1 & 41.48 & 34.87 & 38.88 & 38.41 & 90.98 & 82.37 & 86.97 & 86.77 & 44.89 & 29.57 & 48.76 & 41.07 & 49.00 & 30.90 & 47.00 & 42.30 \\
VideoReward        & 23.45 & 28.86 & -     & 26.16 & 60.32 & 67.74 & -     & 64.03 & 48.74 & 46.92 & -     & 47.83 & 46.36 & 48.31 & -     & 47.34 \\
UnifiedReward      & 25.20 & 27.20 & 22.80 & 25.07 & 71.00 & 64.80 & 68.00 & 67.93 & 53.60 & 42.21 & 53.60 & 49.80 & 58.61 & 43.91 & 53.64 & 52.05 \\
VisionReward       & 41.28 & 33.47 & 35.07 & 36.61 & 87.17 & 84.37 & 82.16 & 84.57 & 43.13 & 41.49 & 37.22 & 40.61 & 46.85 & 45.32 & 38.25 & 43.47 \\
Q-Align            & 28.66 & 28.06 & 27.86 & 28.19 & 75.55 & 69.74 & 68.94 & 71.41 & 45.35 & 25.97 & 33.39 & 34.90 & 54.71 & 34.01 & 37.78 & 42.17 \\
LiFT               & -     & -     & -     & -     & -     & -     & -     & -     & -2.64 & 9.59  & -     & 3.48  & -3.34 & 10.77 & -     & 3.72  \\
AIGVE-MACS         & 20.12 & 12.48 & 14.09 & 15.56 & 62.37 & 46.48 & 45.27 & 51.37 & 24.28 & 13.60 & 12.24 & 16.71 & 27.30 & 6.90  & 13.03 & 15.74 \\
VideoPhy2-AutoEval & -     & 28.46 & 16.23 & 22.35 & -     & 73.75 & 52.31 & 63.03 & -     & 34.35 & 25.17 & 29.76 & -     & 35.42 & 25.41 & 30.42 \\
Dover              & 39.08 & 31.06 & 31.86 & 34.00 & 84.77 & 74.75 & 75.92 & 78.48 & 39.96 & 24.61 & 27.08 & 30.55 & 50.24 & 32.83 & 33.00 & 38.69 \\
\midrule
\multicolumn{17}{c}{\textbf{Ours}} \\ 
\midrule
\score (SFT only) & & & & & & & & & & & & & & & &     \\
\score (RL w/o SFT) & 45.09 & 46.09 & 41.28 & 44.15 & 90.78 & 90.18 & 87.98 & 89.65 & 49.69 & 59.36 & 48.87 & 52.64 & 56.84 & 62.05 & 49.91 & 56.27 \\
\score (SFT $+$ RL) & & & & & & & & & & & & & & & &     \\
$\Delta$ over Best Baseline & & & & & & & & & & & & & & & &     \\
\bottomrule
\end{tabular}
}
\label{tab:4_vs2_bench_all}
\end{table}

==> tables/apdx_full_res_aigve.tex <==
\begin{table}[h]

\small
\centering
\caption{Full evaluation results on \textbf{AIGVE-Bench}. \textbf{Bold} denotes the best model and the \underline{underlined} denotes the second best.}
\scalebox{0.85}{
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc|c|ccc|c|ccc|c}
\toprule

\multirow{2}{*}{\textbf{AIGVE-Bench}} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{Relaxed Accuracy} & \multicolumn{4}{c}{PLCC}  \\  \cmidrule{2-13}
 & Visual  & Align  & Phy  & Avg  
 & Visual  & Align  & Phy  & Avg    
 & Visual  & Align  & Phy  & Avg  \\ 
 \midrule
\multicolumn{13}{c}{\textbf{Reward/Scoring Models for Image}} \\ \midrule
ImageReward        & 26.10 & 27.30 & 31.08 & 28.16 & 65.05 & 61.18 & 31.08 & 52.44 & 14.42  & 16.41 & 5.50  & 12.11 \\
DeQA               & 29.40 & 17.62 & 20.79 & 22.60 & 83.41 & 68.01 & 20.79 & 57.40 & 24.95  & 2.16  & 10.97 & 12.69 \\
Q-Insight          & 29.31 & 21.41 & 21.00 & 23.91 & 84.93 & 82.71 & 21.00 & 62.88 & 26.39  & 17.93 & 16.89 & 20.40 \\
\midrule
\multicolumn{13}{c}{\textbf{Reward/Scoring Models for Video}} \\ 
\midrule
VideoScore-v1.1 & 26.18 & 21.16 & 29.19 & 25.51 & 74.31 & 68.34 & 29.19 & 57.28 & -10.35 & -2.24 & 6.61  & -1.99 \\
VideoReward        & 16.39 & 27.25 & -     & 21.82 & 45.70 & 71.31 & -     & 58.51 & 22.06  & 43.42 & -     & 32.74 \\
UnifiedReward      & 32.65 & \underline{50.23} & \underline{60.77} & 47.88 & 65.38 & 77.23 & \underline{60.77} & 67.79 & 36.65  & 14.59 & 24.01 & 25.08 \\
VisionReward       & \underline{32.69} & 21.28 & 24.00 & 25.99 & \textbf{88.51} & 76.99 & 24.00 & 63.17 & 44.46  & 16.71 & 23.62 & 28.26 \\
Q-Align            & 29.31 & 31.66 & 35.32 & 32.10 & 73.65 & 69.62 & 35.32 & 59.53 & 18.07  & 2.51  & 2.33  & 7.64  \\
AIGVE-MACS         & \textbf{36.27} & \textbf{61.34} & \textbf{62.70} & \textbf{53.44} & 72.21 & \textbf{83.74} & \textbf{62.70} & \textbf{72.88} & 39.55  & 38.71 & 15.91 & 31.39 \\
VideoPhy2-Auto-Eval & -     & 45.82 & 53.36 & \underline{49.59} & -     & \underline{82.75} & 53.36 & \underline{68.06} & -      & 15.83 & 21.59 & 18.71 \\
Dover              & 27.46 & 26.64 & 28.20 & 27.43 & 79.25 & 74.85 & 28.20 & 60.77 & 18.39  & 6.42  & 1.37  & 8.73  \\
\midrule
\multicolumn{13}{c}{\textbf{Ours}} \\ 
\midrule
\score (SFT only) & 29.89 & 34.50 & 40.10 & 34.83 & 76.12 & 79.29 & 40.1  & 65.17 & 16.96  & 25.07 & 10.21 & 17.41 \\
\score (RL w/o SFT) & 28.41 & 18.76 & 20.41 & 22.53 & \underline{85.01} & 78.51 & 20.41 & 61.31 & 23.31  & 32.25 & 15.63 & 23.73 \\
\score (RL + SFT) & 31.00 & 34.34 & 41.88 & 35.74 & 71.02 & 81.84 & 41.88 & 64.91 & 15.60  & 21.25 & 13.23 & 16.69 \\
\bottomrule
\end{tabular}
}

\label{tab:apdx_full_res_aigve}
\end{table}
